Strip-Fusion: Spatiotemporal Fusion for Multispectral Pedestrian Detection

Pedestrian detection is a critical task in robot perception. Multispectral modalities (visible light and thermal) can boost pedestrian detection performance by providing complementary visual information. Several gaps remain with multispectral pedestrian detection methods. First, existing approaches primarily focus on spatial fusion and often neglect temporal information. Second, RGB and thermal image pairs in multispectral benchmarks may not always be perfectly aligned. Pedestrians are also challenging to detect due to varying lighting conditions, occlusion, etc. This work proposes Strip-Fusion, a spatial-temporal fusion network that is robust to misalignment in input images, as well as varying lighting conditions and heavy occlusions. The Strip-Fusion pipeline integrates temporally adaptive convolutions to dynamically weigh spatial-temporal features, enabling our model to better capture pedestrian motion and context over time. A novel Kullback-Leibler divergence loss was designed to mitigate modality imbalance between visible and thermal inputs, guiding feature alignment toward the more informative modality during training. Furthermore, a novel post-processing algorithm was developed to reduce false positives. Extensive experimental results show that our method performs competitively for both the KAIST and the CVC-14 benchmarks. We also observed significant improvements compared to previous state-of-the-art on challenging conditions such as heavy occlusion and misalignment.

==> tables/cvc_14_pp_results.tex <==

\begin{table}[t]
\centering
\caption{\textbf{CVC-14} MR-All results for Algorithm 1 post-processing.
$F$ is the number of frames and $S_T$ the temporal stride. $s^v$ and $s^t$ denote visible and thermal confidence thresholds, and $iou_{\text{thres}}$ the IoU threshold. Scores are fused by AVG, $(s^v+s^t)/2$, or MAX, $\max(s^v,s^t)$. KL divergence uses $\beta=1$. The default setting in the main paper is $s^v=s^t=0.1$, $iou_{\text{thres}}=0.75$, AVG.}
\normalsize
\setlength{\tabcolsep}{3pt}
\begin{tabular}{c c c c c c | c c }
\toprule
F & $S_T$ & $s^v$ & $s^t$ & $iou_{thres}$ & Mode &
\textbf{No KL} & \textbf{With KL}  \\
\midrule
1 & 1 & 0.1 & 0.1 & 0.50 & AVG & 17.90 & 18.94 \\
1 & 1 & 0.1 & 0.1 & 0.50 & MAX & 21.17 & 20.46 \\
1 & 1 & 0.1 & 0.1 & 0.75 & AVG & \textbf{17.79} & \textbf{18.76} \\
1 & 1 & 0.1 & 0.1 & 0.75 & MAX & 20.02 & 20.56 \\
1 & 1 & 0.2 & 0.2 & 0.50 & AVG & 17.88 & 18.96 \\
1 & 1 & 0.2 & 0.2 & 0.50 & MAX & 19.67 & 20.89 \\
1 & 1 & 0.2 & 0.2 & 0.75 & AVG & 17.81 & 18.76 \\
1 & 1 & 0.2 & 0.2 & 0.75 & MAX & 19.30 & 20.56 \\
\midrule
3 & 3 & 0.1 & 0.1 & 0.50 & AVG & 17.93 & 16.72 \\
3 & 3 & 0.1 & 0.1 & 0.50 & MAX & 18.83 & 18.27 \\
3 & 3 & 0.1 & 0.1 & 0.75 & AVG & \textbf{17.26} & 16.53 \\
3 & 3 & 0.1 & 0.1 & 0.75 & MAX & 18.53 & 17.61 \\
3 & 3 & 0.2 & 0.2 & 0.50 & AVG & 18.12 & 16.63 \\
3 & 3 & 0.2 & 0.2 & 0.50 & MAX & 19.40 & 17.67 \\
3 & 3 & 0.2 & 0.2 & 0.75 & AVG & 17.48 & \textbf{16.46} \\
3 & 3 & 0.2 & 0.2 & 0.75 & MAX & 18.70 & 17.39 \\
\midrule
5 & 3 & 0.1 & 0.1 & 0.50 & AVG & 16.89 & 16.41 \\
5 & 3 & 0.1 & 0.1 & 0.50 & MAX & 18.42 & 17.99 \\
5 & 3 & 0.1 & 0.1 & 0.75 & AVG & 16.76 & \textbf{16.34} \\
5 & 3 & 0.1 & 0.1 & 0.75 & MAX & 17.14 & 17.37 \\
5 & 3 & 0.2 & 0.2 & 0.50 & AVG & 16.69 & 16.47 \\
5 & 3 & 0.2 & 0.2 & 0.50 & MAX & 18.28 & 17.67 \\
5 & 3 & 0.2 & 0.2 & 0.75 & AVG & \textbf{16.54} & \textbf{16.34} \\
5 & 3 & 0.2 & 0.2 & 0.75 & MAX & 16.98 & 17.34 \\
\midrule
7 & 3 & 0.1 & 0.1 & 0.50 & AVG & 16.85 & 19.03 \\
7 & 3 & 0.1 & 0.1 & 0.50 & MAX & 18.37 & 20.81 \\
7 & 3 & 0.1 & 0.1 & 0.75 & AVG & 17.09 & \textbf{18.99} \\
7 & 3 & 0.1 & 0.1 & 0.75 & MAX & 17.78 & 19.82 \\
7 & 3 & 0.2 & 0.2 & 0.50 & AVG & \textbf{16.78} & 18.97 \\
7 & 3 & 0.2 & 0.2 & 0.50 & MAX & 17.81 & 20.41 \\
7 & 3 & 0.2 & 0.2 & 0.75 & AVG & 16.97 & 19.01 \\
7 & 3 & 0.2 & 0.2 & 0.75 & MAX & 17.90 & 19.32 \\
\midrule
7 & 5 & 0.1 & 0.1 & 0.50 & AVG & 16.73 & 19.11 \\
7 & 5 & 0.1 & 0.1 & 0.50 & MAX & 17.87 & 19.93 \\
7 & 5 & 0.1 & 0.1 & 0.75 & AVG & 16.80 & 18.82 \\
7 & 5 & 0.1 & 0.1 & 0.75 & MAX & 17.05 & 19.65 \\
7 & 5 & 0.2 & 0.2 & 0.50 & AVG & \textbf{16.68} & 18.88 \\
7 & 5 & 0.2 & 0.2 & 0.50 & MAX & 18.40 & 20.46 \\
7 & 5 & 0.2 & 0.2 & 0.75 & AVG & 16.85 & \textbf{18.69} \\
7 & 5 & 0.2 & 0.2 & 0.75 & MAX & 17.87 & \textbf{18.69} \\
\bottomrule
\end{tabular}
\label{tab:cvc14_algo1_thresholds}
\end{table}


==> tables/cvc_frames_per_sec.tex <==
\begin{table}[h]
\centering
\caption{\textbf{CVC-14} comparison of inference time in frames-per-second for each sequence. Recall the Number of Frames ($F$) and stride ($S_T$).}
\begin{tabular}{c|c|ccc|ccc}
\hline
\multirow{2}{*}{F} & \multirow{2}{*}{S\textsubscript{T}} 
& \multicolumn{3}{c|}{\textbf{No KL} ($\beta = 0$)} 
& \multicolumn{3}{c}{\textbf{With KL} ($\beta = 1$)} \\
\cline{3-8}
 & & Algo. 1 & VIS & IR & Algo. 1 & VIS & IR \\
\hline
1 & 1  & 3.7279 & 3.8658 & 4.1278 & 3.4043 & 4.1462 & 4.1729 \\
3 & 3  & 2.8153 & 2.8694 & 2.8597 & 2.7421 & 2.8676 & 2.8647 \\
5 & 3  & 2.1206 & 2.1933 & 2.2105 & 2.1850 & 2.2049 & 2.2044 \\
7 & 3  & 1.8601 & 1.8709 & 1.8659 & 1.8623 & 1.8709 & 1.8723 \\
7 & 10 & 1.8491 & 1.8766 & 1.8775 & 1.8523 & 1.8684 & 1.8689 \\
\hline
\end{tabular}
\label{tab:cvc14_fps}
\end{table}


==> tables/kaist_frames_per_sec.tex <==
\begin{table}[h]
\centering
\caption{\textbf{KAIST} comparison of inference time in frames-per-second for each sequence. Recall the Number of Frames ($F$) and stride ($S_T$).}
\begin{tabular}{c|c|ccc|ccc}
\hline
\multirow{2}{*}{F} & \multirow{2}{*}{S\textsubscript{T}} 
& \multicolumn{3}{c|}{\textbf{No KL} ($\beta = 0$)} 
& \multicolumn{3}{c}{\textbf{With KL} ($\beta = 2$)} \\
\cline{3-8}
 & & Algo. 1 & VIS & IR & Algo. 1 & VIS & IR \\
\hline
1 & 1  & 3.6599 & 3.3662 & 3.8625 & 3.8023 & 3.3331 & 3.9262 \\
3 & 3  & 2.4697 & 2.5685 & 2.6519 & 2.7125 & 2.7384 & 2.7442 \\
5 & 3  & 1.9156 & 2.0040 & 2.0191 & 2.1030 & 2.1130 & 2.1295 \\
7 & 3  & 1.5997 & 1.6653 & 1.6835 & 1.7666 & 1.7644 & 1.7935 \\
7 & 10 & 1.7508 & 1.7954 & 1.8178 & 1.8312 & 1.8269 & 1.8525 \\
\hline
\end{tabular}
\label{tab:kaist_fps}
\end{table}

==> tables/kaist_pp_results.tex <==
\begin{table}[t]
\centering
\caption{\textbf{KAIST} MR-All results for Algorithm 1 post-processing.
$F$ is the number of frames and $S_T$ the temporal stride. $s^v$ and $s^t$ denote visible and thermal confidence thresholds, and $iou_{\text{thres}}$ the IoU threshold. Scores are fused by AVG, $(s^v+s^t)/2$, or MAX, $\max(s^v,s^t)$. KL divergence uses $\beta=2$. The default setting in the main paper is $s^v=s^t=0.1$, $iou_{\text{thres}}=0.75$, AVG.}
\normalsize
\setlength{\tabcolsep}{3pt}

\begin{tabular}{c c c c c c | c  c}
\toprule
F & $S_T$ & $s^v$ & $s^t$ & $iou_{thres}$ & Mode & \textbf{No KL } & \textbf{With KL} \\
\midrule
1 & 1 & 0.1 & 0.1 & 0.50 & AVG & 9.90 & \textbf{7.40} \\
1 & 1 & 0.1 & 0.1 & 0.50 & MAX & 10.65 & 9.01 \\
1 & 1 & 0.1 & 0.1 & 0.75 & AVG & \textbf{9.69} & 7.52 \\
1 & 1 & 0.1 & 0.1 & 0.75 & MAX & 9.83 & 7.51 \\
1 & 1 & 0.2 & 0.2 & 0.50 & AVG & 10.64 & \textbf{7.40} \\
1 & 1 & 0.2 & 0.2 & 0.50 & MAX & 11.15 & 8.18 \\
1 & 1 & 0.2 & 0.2 & 0.75 & AVG & 10.38 & 7.49 \\
1 & 1 & 0.2 & 0.2 & 0.75 & MAX & 10.83 & 7.54 \\
\midrule
3 & 3 & 0.1 & 0.1 & 0.50 & AVG & 9.92 & 8.11 \\
3 & 3 & 0.1 & 0.1 & 0.50 & MAX & 11.25 & 9.48 \\
3 & 3 & 0.1 & 0.1 & 0.75 & AVG & \textbf{9.84} & \textbf{8.01} \\
3 & 3 & 0.1 & 0.1 & 0.75 & MAX & 10.43 & 8.82 \\
3 & 3 & 0.2 & 0.2 & 0.50 & AVG & 10.31 & 9.02 \\
3 & 3 & 0.2 & 0.2 & 0.50 & MAX & 10.87 & 9.84 \\
3 & 3 & 0.2 & 0.2 & 0.75 & AVG & 10.17 & 8.73 \\
3 & 3 & 0.2 & 0.2 & 0.75 & MAX & 11.15 & 9.67 \\
\midrule
5 & 3 & 0.1 & 0.1 & 0.50 & AVG & 9.05 & \textbf{9.74} \\
5 & 3 & 0.1 & 0.1 & 0.50 & MAX & 10.42 & 9.93 \\
5 & 3 & 0.1 & 0.1 & 0.75 & AVG & \textbf{8.84} & 10.01 \\
5 & 3 & 0.1 & 0.1 & 0.75 & MAX & 9.76 & 10.42 \\
5 & 3 & 0.2 & 0.2 & 0.50 & AVG & 9.74 & 10.41 \\
5 & 3 & 0.2 & 0.2 & 0.50 & MAX & 10.87 & 10.75 \\
5 & 3 & 0.2 & 0.2 & 0.75 & AVG & 9.92 & 10.16 \\
5 & 3 & 0.2 & 0.2 & 0.75 & MAX & 10.83 & 11.02 \\
\midrule
7 & 3 & 0.1 & 0.1 & 0.50 & AVG & 10.44 & 10.70 \\
7 & 3 & 0.1 & 0.1 & 0.50 & MAX & 12.03 & 10.14 \\
7 & 3 & 0.1 & 0.1 & 0.75 & AVG & 10.23 & 9.91 \\
7 & 3 & 0.1 & 0.1 & 0.75 & MAX & \textbf{9.76} & \textbf{9.36} \\
7 & 3 & 0.2 & 0.2 & 0.50 & AVG & 11.23 & 11.60 \\
7 & 3 & 0.2 & 0.2 & 0.50 & MAX & 11.72 & 11.41 \\
7 & 3 & 0.2 & 0.2 & 0.75 & AVG & 10.95 & 11.07 \\
7 & 3 & 0.2 & 0.2 & 0.75 & MAX & 10.72 & 10.16 \\
\midrule
7 & 10 & 0.1 & 0.1 & 0.50 & AVG & 9.38 & 8.84 \\
7 & 10 & 0.1 & 0.1 & 0.50 & MAX & 11.16 & 10.10 \\
7 & 10 & 0.1 & 0.1 & 0.75 & AVG & \textbf{9.33} & 8.40 \\
7 & 10 & 0.1 & 0.1 & 0.75 & MAX & 9.58 & \textbf{8.39} \\
7 & 10 & 0.2 & 0.2 & 0.50 & AVG & 10.28 & 9.51 \\
7 & 10 & 0.2 & 0.2 & 0.50 & MAX & 11.50 & 9.58 \\
7 & 10 & 0.2 & 0.2 & 0.75 & AVG & 10.14 & 9.16 \\
7 & 10 & 0.2 & 0.2 & 0.75 & MAX & 11.11 & 9.37 \\
\bottomrule
\end{tabular}
% }
\label{tab:kaist_algo1_thresholds}
\end{table}
